Bongard-RWR+: Real-World Representations of Fine-Grained Concepts in Bongard Problems

Bongard Problems (BPs) provide a challenging testbed for abstract visual reasoning (AVR), requiring models to identify visual concepts fromjust a few examples and describe them in natural language. Early BP benchmarks featured synthetic black-and-white drawings, which might not fully capture the complexity of real-world scenes. Subsequent BP datasets employed real-world images, albeit the represented concepts are identifiable from high-level image features, reducing the task complexity. Differently, the recently released Bongard-RWR dataset aimed at representing abstract concepts formulated in the original BPs using fine-grained real-world images. Its manual construction, however, limited the dataset size to just $60$ instances, constraining evaluation robustness. In this work, we introduce Bongard-RWR+, a BP dataset composed of $5\,400$ instances that represent original BP abstract concepts using real-world-like images generated via a vision language model (VLM) pipeline. Building on Bongard-RWR, we employ Pixtral-12B to describe manually curated images and generate new descriptions aligned with the underlying concepts, use Flux.1-dev to synthesize images from these descriptions, and manually verify that the generated images faithfully reflect the intended concepts. We evaluate state-of-the-art VLMs across diverse BP formulations, including binary and multiclass classification, as well as textual answer generation. Our findings reveal that while VLMs can recognize coarse-grained visual concepts, they consistently struggle with discerning fine-grained concepts, highlighting limitations in their reasoning capabilities.

==> figures/cs-d1s-i1s-d1s_concept-groups_proprietary-models.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{images/rwr-plus-i1s-d1s-concept-groups-closed-models}
    \caption{\textbf{Proprietary model performance across concept groups.} Results on \rwrp in the CS ($K=16$), D1S, and I1S tasks is presented.}
    \label{fig:rwr-plus-cs-d1s-i1s-concept-groups-proprietary-models}
\end{figure}


==> figures/mc-selection-concept-groups.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/mc-selection-rwr-plus-concept-groups.png}
    \caption{\textbf{Concept Selection.} Model performance in the CS task for $K \in \{2, 4, 8, 16\}$ (x-axis). Performance decreases across all concept groups, though the accuracy on Size and Branching shows the smallest decline.
    {\color{red}DEPRECATED: Please use the wrapped figure in experiments.tex}}
    \label{fig:rwr-plus-mc-seletion-concept-groups}
\end{figure}


==> figures/rwr-plus-all-strategies.tex <==
\begin{table}[t]
\centering
\caption{{\color{red}DEPRECATED: Please use Table~\ref{tab:rwr-plus-i1s-i2s-d1s-d2s} in experiments.tex}}
% \label{tab:rwr-plus-i-i-i1s}
\begin{tabular}{lcccc}
\toprule
 & D1S & D2S & I1S & I2S \\
\midrule
DeepSeek R1 70B & 0.57 & 0.56 & - & - \\
InternVL2.5 78B & 0.57 & - & 0.50 & 0.39 \\
LLaVa-Next 110B & 0.54 & - & 0.50 & 0.50 \\
MiniCPM-o 2.6 8B & 0.51 & - & 0.48 & 0.45 \\
Qwen2-VL 72B & 0.58 & - & 0.49 & 0.44 \\
Similarity Classifier & - & - & 0.52 & 0.54 \\
\bottomrule
\end{tabular}
\end{table}


==> figures/rwr-plus-d1s.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/rwr-plus-d1s.png}
    \caption{Model accuracy in the Description-to-Side experiment. The X-axis shows the models used as solvers, while the Y-axis shows the models used to generate the descriptions.
    {\color{red}DEPRECATED: Please use the wrapped figure in experiments.tex}
    }
    % \label{fig:rwr-plus-d1s}
\end{figure}

==> figures/rwr-plus-gs-mc-selection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/rwr-plus-gs-mc-selection.png}
    \caption{\textbf{Grey-scale \rwrp.} The impact of using greyscale images on accuracy in the CS task for $K \in \{2, 4, 8, 16\}$ (x-axis).
    % The X-axis indicates the number of candidate concepts among which the model must identify the one matching the BP.
    Differences in accuracy are shown using lighter colors and are annotated above the corresponding bars.
    {\color{red}DEPRECATED: Please use ablation-greyscale-size.tex}
    }
    % \label{fig:rwr-plus-gs-mc-selection}
\end{figure}

==> figures/rwr-plus-i-i-d1s.tex <==
\begin{table}[t]
\centering
\caption{Results of the Description-To-Side experiment across dataset variants with varying numbers of images per side.
{\color{red} DEPRECATED: Please use rwr-plus-i-i.tex.}
}
% \label{tab:rwr-plus-i-i-d1s}
\begin{tabular}{lccccc}
\toprule
 & DeepSeek-R1 70B & InternVL2.5 78B & LLaVa-Next 110B & MiniCPM-o 2.6 & Qwen2-VL 72B \\
\midrule
RWR+ 2-2 & 0.56 & 0.56 & 0.53 & 0.50 & 0.55 \\
RWR+ 3-3 & 0.62 & 0.60 & 0.56 & 0.51 & 0.58 \\
RWR+ 4-4 & 0.64 & 0.61 & 0.58 & 0.54 & 0.63 \\
RWR+ 5-5 & 0.64 & 0.62 & 0.57 & 0.52 & 0.60 \\
RWR+ 6-6 & - & - & - & 0.53 & - \\
\bottomrule
\end{tabular}
\end{table}


==> figures/rwr-plus-i-i-i1s.tex <==
\begin{table}[t]
\centering
\caption{Results of the Image-To-Side experiment across dataset variants with varying numbers of images per side.
{\color{red} DEPRECATED: Please use rwr-plus-i-i.tex.}
}
% \label{tab:rwr-plus-i-i-i1s}
\begin{tabular}{lcccc}
\toprule
 & InternVL2.5 78B & Qwen2-VL 72B & LLaVa-Next 110B & MiniCPM-o 2.6 \\
\midrule
RWR+ 2-2 & 0.51 & 0.51 & 0.49 & 0.50 \\
RWR+ 3-3 & 0.54 & 0.54 & - & 0.51 \\
RWR+ 4-4 & 0.54 & 0.54 & - & 0.51 \\
RWR+ 5-5 & 0.54 & 0.55 & 0.51 & 0.52 \\
RWR+ 6-6 & 0.55 & - & - & 0.51 \\
\bottomrule
\end{tabular}
\end{table}


==> figures/rwr-plus-i1s-concept-groups.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/rwr-plus-i1s-concept-groups.png}
    \caption{Models' performance in the Image-to-Side experiment across distinct concept groups in RWR+ 6-6. Although all models achieve an average score equivalent to random guessing, their performance varies notably across different groups.}
    \label{fig:rwr-plus-i1s-concept-groups}
\end{figure}

==> figures/rwr-plus-mc-selection-param-scaling.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/rwr-plus-mc-selection-param-scaling.png}
    \caption{Accuracy of models of varying sizes on the Concept Selection experiment for $C=16$. The X-axis denotes the number of model parameters, and the Y-axis indicates classification accuracy. Performance consistently improves with larger model sizes.
    {\color{red}DEPRECATED: Please use ablation-greyscale-size.tex}}
    % \label{fig:rwr-plus-mc-selection-param-scaling}
\end{figure}

==> figures/rwr-plus-mc-selection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/rwr-plus-mc-selection}
    \caption{\textbf{Concept Selection.} Model accuracy in the CS task for $K \in \{2, 4, 8, 16\}$ (x-axis).
    % The X-axis indicates the number of candidate concepts among which the model must identify the one matching the BP.
    Accuracy declines as the number of candidate concepts increases.
    {\color{red}DEPRECATED: Please use wrapped figure in experiments.tex}}
    % \label{fig:rwr-plus-mc-selection}
\end{figure}


==> figures/similarity-vs-accuracy.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/similarity_vs_accuracy}
    \caption{
    \textbf{The impact of the test image similarity on model performance.} The x-axis shows the difference between each test image's similarity to the right side of the problem and its similarity to the left side.
    }
    \label{fig:rwr-plus-mc-selection-concept-groups}
\end{figure}


==> sections/plans.tex <==
\section{Description of experiments -- TO BE REMOVED}

\paragraph{Concept selection.}
We formulated a task in which the model had to select the concept matching the BP from a set of provided choices.
We considered $C \in \{2, 4, 8, 16\}$.

Experiment: Main
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 6-6
Number of concepts: 2, 4, 8, 16
Total number of runs: 4 models x 4 concepts => 16
Priority: {\color{red}High}
State: {\color{green}Ready}

Experiment: How does the number of images per side impact model performance? Images are arranged to maximally utilize the available space
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 1-1,  RWR+ 2-2,  RWR+ 3-3,  RWR+ 4-4,  RWR+ 5-5
Number of concepts: 16
Total number of runs: 4 models x 5 datasets => 20
Priority: {\color{blue}Low}
State: {\color{green} Done}
Decision: Doliczyć dla 5

\paragraph{Image to Side (I1S).}

Experiment: Main
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 6-6
Matrix side layout: 3x2 (3 rows by 2 columns)
Total number of runs: 4 models => 4
Priority: {\color{red}High}
State: {\color{green}Ready}

Experiment: How does the number of images per side impact model performance? Images are arranged to maximally utilize the available space
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 1-1,  RWR+ 2-2,  RWR+ 3-3,  RWR+ 4-4,  RWR+ 5-5
Matrix side layouts: 1x1, 2x1, 3x1, 2x2, 3x2 with one missing
Total number of runs: 4 models x 5 datasets => 20
Priority: {\color{orange}Medium}
State: {\color{green}Ready}

Experiment: How does the number of images per side impact model performance? Ablation, where images are arranged following the original 3x2 layout.
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 1-1,  RWR+ 2-2,  RWR+ 3-3,  RWR+ 4-4,  RWR+ 5-5
Matrix side layout: 3x2
Total number of runs: 4 models x 5 datasets => 20
Priority: {\color{blue}Low}

\paragraph{Description to Side (D1S).}

Experiment: Generate descriptions, both for D1s and D2s
Description models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+
Total number of runs: 4 models => 4
Priority: {\color{red}High}
State: {\color{green}Ready}

Experiment: Main
Description models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Prediction models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B), and DeepSeek-R1-Distill-Qwen-32B
Datasets: RWR+ 6-6
Total number of runs: 4 description models x 5 prediction models => 20
Priority: {\color{red}High}
State: {\color{green}Ready}

Experiment: How does the number of descriptions per side impact model performance?
Description models: InternVL2.5 (78B) (Let's limit this to a single description model, we can select one that works best in the Main D1S experiment)
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B), and DeepSeek-R1-Distill-Qwen-32B
Datasets: RWR+ 1-1,  RWR+ 2-2,  RWR+ 3-3,  RWR+ 4-4,  RWR+ 5-5
Total number of runs: 5 models x 5 datasets => 25
Priority: {\color{orange}Medium}
State: {\color{green}Ready}

\paragraph{Images to Sides (I2S).}

Experiment: Main
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 6-6
Matrix side layout: 3x2 (3 rows by 2 columns)
Total number of runs: 4 models => 4
Priority: {\color{red}High}
State: {\color{green}Ready}
Decision: Wstawiamy wyniki dla 4 klas

Experiment: How does the number of images per side impact model performance? Images are arranged to maximally utilize the available space
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Datasets: RWR+ 1-1,  RWR+ 2-2,  RWR+ 3-3,  RWR+ 4-4,  RWR+ 5-5
Matrix side layouts: 1x1, 2x1, 3x1, 2x2, 3x2 with one missing
Total number of runs: 4 models x 5 datasets => 20
Priority: {\color{orange}Medium}

\paragraph{Descriptions to Sides (D2S).}

Experiment: Main
Description models: InternVL2.5 (78B) (Let's limit this to a single description model, we can select one that works best in the Main D1S experiment)
Prediction models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B), and DeepSeek-R1-Distill-Qwen-32B
Datasets: RWR+ 6-6
Total number of runs: 5 prediction models => 5
Priority: {\color{red}High}
State: {\color{green}Ready}

Experiment: How does the number of descriptions per side impact model performance?
Description models: InternVL2.5 (78B) (Let's limit this to a single description model, we can select one that works best in the Main D1S experiment)
Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B), and DeepSeek-R1-Distill-Qwen-32B
Datasets: RWR+ 1-1,  RWR+ 2-2,  RWR+ 3-3,  RWR+ 4-4,  RWR+ 5-5
Total number of runs: 5 models x 5 datasets => 25
Priority: {\color{orange}Medium} 
EST: 3.5 days

\subsection{Ablations}

\paragraph{How important is the image color?}

Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Tasks: I1S RWR+ 6-6, I1S RWR+ 3-3, I2S RWR+ 6-6, I2S RWR+ 3-3, Concept selection with $C=16$ RWR+ 6-6
Alternative task: Image-To-Side
Total number of runs: 4 models x 5 tasks => 20
Priority: {\color{red}High}
% State: {\color{green}Ready}
Decision: i1s w appendix tylko dla bazowego zbioru RWR+
State: {\color{green}Ready}

\paragraph{How important is the model size?}

Idea: Let's take an experiment where models achieve relatively high scores (definitely distinguishable from random guessing). Ideally this could be I1S or D1S, but if model performance is insufficient, then let's use Concept selection with $C = 16$.
Models: InternVL2.5: 78B, 38B, 26B, 8B; Qwen2-VL: 72B-Instruct, 7B-Instruct; LLaVa-NeXT: 110B, 72B, 32B (Qwen), 8B (llama 3)
Datasets: RWR+ 6-6
Number of concepts: 16
Total number of runs: 4 intern + 2 qwen + 4 llava - 3 (as the biggest models will be already evaluated) => 7
Priority: {\color{red}High}
State: {\color{green}Ready}

\paragraph{Answer bias}

Models: InternVL2.5 (78B), Qwen2-VL (72B-Instruct), LLaVa-NeXT (110B), and MiniCPM-o-2.6 (8B)
Tasks: I1S
Datasets: RWR+ 6-6
Prompts: 1 example: LEFT-RIGHT, 2 examples: LEFT-RIGHT and RIGHT-LEFT, 2 examples: RIGHT-LEFT and LEFT-RIGHT
Total number of runs: 4 models x 3 prompts => 12
Priority: {\color{red}High}
State: {\color{yellow}In progress}

\paragraph{Real vs. generated images}
TODO: Extend Concept Selection to more classes
Tasks: 
Datasets: RWR and RWR+ less than 6 images per side
State: {\color{yellow}In progress}

\paragraph{NLP metrics on predicted concepts}
TODO


==> tables/concept-generation_rwrp-openworld.tex <==
\addtolength{\tabcolsep}{-1pt}
\begin{table}[t]
\centering
\small
\caption{
\textbf{Concept Generation: \rwrp vs. \openworld.}
Image-based: The results on \rwrp come from \cpmb. The results on \openworld come from GPT-4V.
Text-based: The results on \rwrp come from \qwenb. The results on \openworld come from ChatGPT + BLIP-2 w/ Fine-tuning.
}
\label{tab:concept-generation-rwrp-vs-openworld}
\begin{tabular}{lcccccccccc}
\toprule
 & \multicolumn{5}{c}{Image} & \multicolumn{5}{c}{Text} \\
 \cmidrule{2-6} \cmidrule{7-11}
 & $\text{BLEU}_1$ & $\text{BLEU}_2$ & METEOR & $\text{ROUGE}_L$ & CIDEr & $\text{BLEU}_1$ & $\text{BLEU}_2$ & METEOR & $\text{ROUGE}_L$ & CIDEr \\
\midrule
\rwrp & $0.077$ & $0.008$ & $0.063$ & $0.181$ & $0.004$ & $0.132$ & $0.021$ & $0.066$ & $0.161$ & $0.018$ \\
\openworld & $0.190$ & $0.073$ & $0.111$ & $0.188$ & $0.527$ & $0.441$ & $0.292$ & $0.222$ & $0.417$ & $1.714$ \\
\bottomrule
\end{tabular}
\end{table}
\addtolength{\tabcolsep}{1pt}


==> tables/proprietary-models.tex <==
\addtolength{\tabcolsep}{-3pt}
\begin{wraptable}[8]{r}{0.425\textwidth}
% \vspace{-10pt}
\centering
\small
\caption{\textbf{Performance of proprietary models on \rwrp.}}
\label{tab:proprietary-models}
{\color{blue}\begin{tabular}{lccc}
\toprule
Model & I1S & D1S & CS, $K=16$ \\
\midrule
Gemini 2.5 Pro & $\textbf{0.65}$ & $\textbf{0.70}$ & $\textbf{0.82}$ \\
GPT 5.1 & $0.65$ & $0.67$ & $0.81$ \\
Claude Sonnet 4.5 & $0.63$ & $0.67$ & $0.76$ \\
\bottomrule
\end{tabular}}
\end{wraptable}
\addtolength{\tabcolsep}{3pt}
